A Dual-Critic Reinforcement Learning Framework for Frame-level Bit Allocation in HEVC/H.265

This paper introduces a dual-critic reinforcement learning (RL) framework to address the problem of frame-level bit allocation in HEVC/H.265. The objective is to minimize the distortion of a group of pictures (GOP) under a rate constraint. Previous RL-based methods tackle such a constrained optimization problem by maximizing a single reward function that often combines a distortion and a rate reward. However, the way how these rewards are combined is usually ad hoc and may not generalize well to various coding conditions and video sequences. To overcome this issue, we adapt the deep deterministic policy gradient (DDPG) reinforcement learning algorithm for use with two critics, with one learning to predict the distortion reward and the other the rate reward. In particular, the distortion critic works to update the agent when the rate constraint is satisfied. By contrast, the rate critic makes the rate constraint a priority when the agent goes over the bit budget. Experimental results on commonly used datasets show that our method outperforms the bit allocation scheme in x265 and the single-critic baseline by a significant margin in terms of rate-distortion performance while offering fairly precise rate control.

==> Makefile <==
FILENAME = dcc_paper
PS_FILE = $(FILENAME).ps
PDF_FILE = $(FILENAME).pdf

# PAPERSIZE = a4
PAPERSIZE = letter

LATEX_FILES = *.dvi *.log *.toc *.tof *.aux *.blg *.lof *.lot *.bbl
CLEAN_FILES = $(LATEX_FILES) *.bak core $(PS_FILE) $(PDF_FILE)
COMPRESS_FILES = *.tex *.bib *.sty *.eps *.ps *.fig *.m *.txt *.pgm *.bst *.cls
UNCOMPRESS_FILES = *.Z *.gz

COMPRESS_DIRS = . Tables Figures
COMPRESS = gzip -q
UNCOMPRESS = gunzip

all: main


main:
	latex main
	@if grep "Warning: Citation" main.log; then bibtex main; \
	latex main; fi;
	@while grep Rerun main.log; do latex main; done;

ps: main
	dvips -t $(PAPERSIZE) -o $(PS_FILE) main

pdf: main
	dvips -t $(PAPERSIZE) -Ppdf -j0 -G0 -o $(PS_FILE) main
	ps2pdf -sPAPERSIZE=$(PAPERSIZE) \
		-dPDFSETTINGS=/prepress \
		-dCompatibilityLevel=1.7 \
		$(PS_FILE) $(PDF_FILE)

clean:
	@for i in $(COMPRESS_DIRS) ; \
	do \
	(if (test -d $$i) ; \
	then cd $$i ; \
	echo "Cleaning $$i" ; \
	rm -f *~ ; \
	rm -f $(CLEAN_FILES) ; \
	fi) \
	done


==> Related.tex <==
\section{Review of RL-based Frame-level Bit Allocation}
\label{sec:prior}
This section briefly reviews the RL approach to frame-level bit allocation in \cite{chen2018reinforcement}, to ease the understanding of the novelty of our proposed method. As depicted in Fig.~\ref{}, 

provides a reinforcement learning framework solution for frame-level bit allocation through deep deterministic policy gradient (DDPG) \cite{lillicrap2015continuous} algorithm. In their work, the RL agent predicts the quantization parameter (QP) of each frame in a GOP as action. To achieve constrained optimization, They define the immediate reward function as:

\begin{equation}
\label{eq:chen}
r_i = -1 \times \frac{D_i}{D_{norm}} -  \lambda \times \frac{R_{target} - R_{encode}}{R_{target}}
\end{equation}
where $D_i$ is the distortion of current frame $i$, $D_{norm}$ is the distortion of the sequence, $R_{target}$ and $R_{encode}$ are the target bit and total encoded bits, and $\lambda$ is the hyper-parameter. 

The first term of eq. (\ref{eq:chen}) is the distortion term calculating the mean square error of each decoded frame. Since the distortion value of dynamic sequences is inherently larger than the distortion value of static sequences, it could cause the learning algorithm to focus more on the dynamic videos. To this end, they add a normalization term $D_{norm}$ to overcome the imbalanced distortion value between dynamic and static videos. The second term of eq. (\ref{eq:chen}) is the rate term, different from the distortion, the rate term only exists when the terminal state is reached. In order to achieve better bit accuracy, in their design, the RL episode reaches its terminal state once the encoding bits is greater than the target bit. The following frames that haven't been encoded yet will be encoded by the QP value equals the QP of I-frame plus 10. And the distortion of those frames will be added as immediate reward of the terminal state.



\begin{comment}
Zhou et al. [] also predicts the QP for each frame as action but use different design of reward function. Their reward function is defined as:
\begin{equation}
\label{eq:zhou}
\begin{split}
&r_i = \alpha_i \times \beta_i \times \gamma_i \\ 
&\alpha_i = \frac{1}{D_i^{\lambda_{1}}} \\ 
&\beta_i = \frac{1}{(D_i - D_{prev})^{\lambda_{2}}} \\ &\gamma_i = \frac{1}{((T_i \times N_i) - \sum_{i=1}^{N_i}R_i)^{\lambda_3}}. 
\end{split}
\end{equation}
where $D_i$ is the distortion of current frame $i$, $D_{prev}$ is the average distortion of previous frames, $T_i$ is the target average number of bit per frame, $N_i$ is the order of current frames, $R_i$ is the encoding bits of current frame, and $\lambda_1$ to $\lambda_3$ are the hyper-parameters. The $\alpha$ term is the distortion term, the $\beta$ term is to regularize the quality consistency in the temporal dimension, and the $\gamma$ term is the rate term. Different from Chen et al. [] that the rate reward only exists at the final step, Zhou et al. [] forces the encoding bit of every frame to be equalized. Therefore, their reward design is only suitable for the constant bit-rate so that they train and test on LDP with small GOP size.
\end{comment}
